SAGA: A Participant-specific Examination of Story Alternatives and Goal Applicability for a Deeper Understanding of Complex Events

Interpreting and assessing goal driven actions is vital to understanding and reasoning over complex events. It is important to be able to acquire the knowledge needed for this understanding, though doing so is challenging. We argue that such knowledge can be elicited through a participant achievement lens. We analyze a complex event in a narrative according to the intended achievements of the participants in that narrative, the likely future actions of the participants, and the likelihood of goal success. We collect 6.3K high quality goal and action annotations reflecting our proposed participant achievement lens, with an average weighted Fleiss-Kappa IAA of 80%. Our collection contains annotated alternate versions of each narrative. These alternate versions vary minimally from the "original" story, but can license drastically different inferences. Our findings suggest that while modern large language models can reflect some of the goal-based knowledge we study, they find it challenging to fully capture the design and intent behind concerted actions, even when the model pretraining included the data from which we extracted the goal knowledge. We show that smaller models fine-tuned on our dataset can achieve performance surpassing larger models.

==> acl_templ.tex <==
\begin{abstract}
This document is a supplement to the general instructions for *ACL authors. It contains instructions for using the \LaTeX{} style files for ACL conferences. 
The document itself conforms to its own specifications, and is therefore an example of what your manuscript should look like.
These instructions should be used both for papers submitted for review and for final versions of accepted papers.
\end{abstract}

\section{Introduction}

These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{acl.tex}),
the \LaTeX{} style file used to format it (\texttt{acl.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
\citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.


==> sections/acknowledgements.tex <==
%\section{Acknowledgments}
%We would like to thank Sayontan Ghosh for providing us with valuable insights into counterfactual stories and the PASTA dataset before leaving for his internship at Amazon.  We value his suggestions and help with HIT evaluations during data collection. We are grateful to Niranjan Balasubramanian for valuable insights into evaluating GPT3.5 and GPT4 models before leaving for his Sabattical at ?? in South Korea.  We thank our amazing crowdworkers for provding several rounds of annotations and evaluations until we found the most suitable setting. 

==> sections/cutouts.tex <==
\textbf{Actual Story:}
1. Jimmy went canoeing with his best friend Carl.
2. Jimmy's mother told him to wear a life vest.
3. Jimmy ignored her advice, and didn't wear one.
4. Jimmy fell out of the boat, and almost drowned.
5. From then on, Jimmy listened to his mother.
\end{quote}
 \begin{figure}
    \centering     \includegraphics[trim=0 .2in 0 0,  width=.9\textwidth]
    {sections/figures/goal-state_fig_v1.png}
    \vspace{-35mm}
	\caption{A Change in a participant's state leads to a counterfactual story situation changing the participant's and other participants' goal achievement. %
 }
	\label{fig:fig1}
 \vspace{-5mm}
\end{figure}
We can infer that Jimmy's goal is ``to go canoeing without any incidents.'' Consider the alternate situation below (a counterfactual story from PASTA~\cite{ghosh2023pasta}) where Jimmy's goal is unchanged, albeit, with a slightly different set of actions.   

\begin{quote} 
\small
\textbf{Counterfactual Story:}
1. Jimmy went canoeing with his best friend Carl.
2. Jimmy's mother told him to wear a life vest.
3. Jimmy ignored her advice, and didn't wear one.
4. Jimmy fell out of the boat, and almost drowned.
5. Jimmy continued to go without a life vest.

\end{quote}
From this counterfactual story we understand the implied state that Jimmy did not learn from his previous fall.  While this state did not affect the participant's goal, if the last sentence was As illustrated in \cref{fig:fig1}, the state change affects the goal achievement of the participant in this counterfactual story.
In the counterfactual Jimmy may not achieve his goal which can affect his mother's goal achievement of "wanting her son's safety".  Knowledge of goals and the conditions that influence them can help a participant revise their plan to change their achievement.  For example, noticing that the currents are rapid Jimmy can wear an emergency life vest on his canoe.   


%\paragraph{Coherence:}  Measures how many of the participant's actions in the story are covered by the goal.   High coherence indicates that all actions are aimed at achieving the described goal.   Low coherence indicates only some of the actions are aimed at achieving the goal.%\paragraph{Explain-abiliy Coverage:} Measures how much of the goal can be explained by the participant's actions.  High coverage indicates the goal can be fully explained by the actions. Low coverage indicate the goal cannot be fully explained by the actions.%\paragraph{Means-end Clarity:} Measures whether the goal description asserts a clear and rational means-end belief explanation of the participant's intention. High clarity indicates a clear unconditional goal that the participant believes can be achieved~\cite{Grice1971-GRIIAU} regardless of the actual outcome.  




%\subsection{Goal Parameters}
%From the story context we can identify the goal dimensions relating to content and intensity:  the difficulty of the goal, a participant's commitment, influence from external factors, state of success, whether the participant would consider a revision and the participant's satisfaction.  Thus we collect the following goal dimensions for each super-ordinate goal: 

%\paragraph{Goal Difficulty $GD_i$:}
%The story context give an indication of the participant's thoughts on the difficulty of achieving their goal.  If this information cannot be inferred from the story, this value is based on an annotator's external knowledge about how difficult the abstract goal achievement will be.  \textit{Possible values of $GD_i$ are: Very Easy, Somewhat Easy, Unsure, Somewhat Difficult, Very Difficult}.

%\paragraph{Goal Commitment $GC_i$:}
%The story context indicates how committed the participant is to achieving their goal.  If this information cannot be inferred from the story, this value is based on an annotator's external knowledge of the commitment required for achieving the abstract goal.  \textit{Possible values of $GC_i$ are: Very High, Somewhat High, Unsure, Somewhat Low, Very Low}.

%\paragraph{Goal Cooperation $GCP_i$:}
%Story events not in the participant's control could assist or hinder the achievement of a participant's goal.  The cooperation or conflict a participant experiences as inferred from the story events is captured by this value. \textit{Possible values of $GI_i$ are: Active Cooperation, Passive Cooperation, None, Passive Conflict, Active Conflict}.

%\paragraph{Goal Conflict $GCP_i$:}
%Story events not in the participant's control could assist or hinder the achievement of a participant's goal.  The cooperation or conflict a participant experiences as inferred from the story events is captured by this value. \textit{Possible values of $GI_i$ are: Active Cooperation, Passive Cooperation, None, Passive Conflict, Active Conflict}.

\paragraph{Goal-State pairs $G^p_i, PS^p_i$:}
Since we want to track the influence of a state change on goal achievement, using a second HIT, for each story $S^p(=S)$, we collect which goals of a participant are also applicable to the corresponding counterfactual stories and whether the goals are achieved in the story.  To measure \textit{presupposition bias}, we ask if the story makes sense and identify the sentences that lead to confusion.   

\paragraph{Goal Achievement based on State:}
For the goals that are not successful in the above HIT we use a third HIT and verify if the Next Action, $N_{ik}$ collected for assessing the goal $G^p$ (where $G^p$=$G_{ik}$) can be used for assessing goal direction in the counterfactual story.  When it can be used we denote it as $NA^p$, otherwise, we obtain a modified Next Action, $NA^{p'}$.  We also obtain annotations for Goal Success, $GS^{p'}_i$, Goal Direction, $GD^{p'}_i$, Goal Revision $GS^{p'}_i$ which apply to the counterfactual story, $S^{p'}$, using either the original or modified Next Action, $NA^p$ or $NA^{p'}$.  For the actual story $S^p$, we denote the Goal Success $GS_{ik}$ as $GS^p$, Goal Direction $GD_{ik}$ as $GD^p$ and Goal Revision $GR_{ik}$ as $GR^p$.  

%\subsection{Crowd Vs AI Annotations}
%\label{sec:Crowd_vs_AI}
%To decide whether to collect annotations from crowd workers on Amazon Mechanical Turk (AMT) or employ an AI model (specifically GPT3.5), we obtained 3 goal annotations from each of the two sources to explain a participant's actions in 250 stories (=6 annotations for a equal number of Newswire and ROC stories).  We designed a human intelligence task (HIT) for collecting crowd annotations and a prompt collecting GPT3.5 annotations for a participant's goal given a story in which the participant mentions are highlighted.  More on the HIT and prompts details are discussed in \cref{sec:HIT_Prompt}.
 
%We validated the collected annotations using the goal evaluation criteria in \cref{sec:Evaluation_Criteria} using 3 crowd workers.  We noticed that the nature of the stories and the task steps elicit a variation in the text style and format, even from the same worker. As expected crowd produced more nuanced goal annotations as shown in table ... when compared to model annotations~\cite{Holtzman2020The,Welleck2020Neural}.  Because model generated content could already contain and lead to misinterpreting reality based on reinforced beliefs~\cite{shumailov2023curse} we decided to obtain annotations from crowd workers. 

%In this initial collection we focused on annotations for a single participant in a story.   We prompted GPT3.5 (text-davinci-003) model to obtain the same 10 annotations. More on the prompts used and HIT details are discussed in \cref{sec:HIT_Prompt}

%Knowledge distillation~\cite{Model_compression,hinton2015distilling,west2022symbolic} has been shown to produce effective task-specific models using knowledge collected from a capable larger model. 
%Crowd workers improved the quality of symbolic knowledge collected from larger models ~\cite{Wiegreffe2021ReframingHC,liu2022wanli} reducing repetition~\cite{Geirhos_2020}, reporting~\cite{gordon2013reporting} and annotator~\cite{geva-etal-2019-modeling,gururangan-etal-2018-annotation}  biases. 
%Evaluating annotations from crowd workers and instruction finetuned language models FlanT5 (xxl-model) and GPT3.5 (text-davinci-003) ~\cite{wei2022finetuned,chung2022scaling,ouyang2022training}
%that are both  that perform well on reasoning in unseen tasks  
%we found  reinforcement learning from human feedback (RLHF)~\cite{ouyang2022training} is better at goal reasoning (discussed in \cref{sec:initial_annotations}).  We leverage the human likability of language scaffolding \cite{clark-etal-2021-thats} and use GPT3 generations as assists for crowd workers to produce more elaborate and nuanced annotations.  

\includegraphics[trim=0 .2in 0 0,  width=.95\linewidth]
     {sections/figures/goal-state_fig3_v2.png}
	\caption{Our approach to modeling the interaction between states that affect a participant's goals and the outcome of such interaction.%
 }
 \vspace{-5mm}
	\label{fig:fig3}
\end{figure*}

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
 \hline
 Model  & Rou & ME &\multicolumn{5}{|c|}{Human Eval}\\ 
  Type  &   L & TR & Cohere & Explain & Faith & Truth & Intent\\
 \hline

\multicolumn{3}{|l|}{Ref mean vals (var < \%) }&4.61&4.54&4.68&4.73&4.39 \\ 
% Ref    &&      &4.64 &4.53 &4.71 &4.77 &4.34 \\
 fT5b   (3-shot) &.42&.40&\underline{3.91}&\underline{4.12}&\underline{4.32} &\underline{4.22}&\underline{3.74} \\
% Ref    &&      &4.64 &4.57 &4.69 &4.78 &4.37 \\
 fT5xxl (3-shot)&.50&.49&\underline{4.35} &4.50 &4.71 &4.66 &\underline{4.00} \\
% Ref    &&      &4.63 &4.52 &4.68 &4.72 &4.42 \\
 gpt3.5t (3-shot)&.44&.52&\underline{4.39} &4.44 &4.83&4.69&\underline{3.83} \\
% Ref    &&      &4.58 &4.57 &4.71 &4.71 &4.27 \\
 gpt4  (3-shot) &.53&.55&\underline{4.35}&\underline{4.31} &4.77 &4.74 &\underline{3.87}\\
\hline
%T511b   &.14&.28&&&&& \\
% Ref    &&      &4.60 &4.60 &4.63 &4.72 &4.52 \\
T5b-ft (0-shot)   &.32&.26&\underline{3.82}&\underline{3.86}&\underline{4.03}&\underline{3.99}&\underline{3.63} \\
fT5b-ft (0-shot)&.3 &.31 &\underline{3.71}&\underline{3.74} &\underline{3.93} &\underline{3.94}&\underline{3.65} \\
% Ref    &&      &4.64 &4.53 &4.71 &4.77 &4.34 \\
fT5b-ft (3-shot)  &.50&.45&4.41&4.39&4.57&4.56&4.29 \\
\hline
\end{tabular}
}
 
 \caption{Evaluation of model generated goals for a volitional participant in \textbf{actual stories}.   Scores underlined are significantly lower than reference scores.  See  \cref{sec:goal_eval} for details on Coherence, Explainability, Faithfulness, Truthfulness and Intentionality; \cref{tab:goal-manual-metrics} \& \ref{tab:goal-automated-metrics} for additional models, metrics and goals in alternative stories.
}
\label{tab:actual-goal-manual-metrics}
\vspace{-5mm}
\end{table}


==> sections/disclaimer.tex <==


\section*{Disclaimer}
\begin{enumerate}
\item 
\item All collected annotations were verified using random manual checks and automated filters  to ensure the annotations do not contain any risky or unsafe words, phrases or sentences. 
%\item We believe there are no risks associated with our work other than the items addressed in the limitations. 
\end{enumerate}

==> sections/inferences.tex <==
\section{Goal Knowledge based Inferences }
\label{sec:Inferences}
Goal annotations in our dataset mostly consist of implied (not stated in the story) information based on commonsense knowledge and world knowledge.  Although, we compute automated metrics listed in \cref{sec:metrics}, we mainly rely on human evaluation using the criteria in \cref{sec:def} when comparing model results.  When there is no easy baseline to compare with in our benchmarking, we compare with the GPT3.5. 

\paragraph{\textit{Goal descriptions are diverse.}}
Based on a reader's bias of the events they think as important, goal descriptions from multiple human annotators point to diverse goals in some situations.  In the collected annotations, 50\% of the story contexts lead to goal descriptions that describe slightly to vastly different goals.  Here we compare how diverse goals from models are.  

\paragraph{\textit{Overarching goals are applicable in diverse situations.}} Most of the goal descriptions are applicable to counterfactual stories.  Only 15\% of the goals are not applicable and this happens when the goals are not overarching and find other reasons.

\paragraph{\textit{State changes affect goal success.}}  A state change in an actual story leading to a counterfactual story can flip the goal success.  This happens in x\% of the situations where an unsuccessful goal is achieved with the state change and in y\% of the situations an achievable goal can no longer be achieved.  There are 2 cases leading to 4 combinations to look into:  1) where the state affects the goal  2) where the state does not affect the goal but a change in situation affects the goal  

\paragraph{\textit{Counterfactual stories do not always make sense.}}  Annotations indicate that 13\% of the stories do not make sense.  However, regardless of whether the story makes sense, human annotators are able to judge whether the goal applies to the counterfactual situation.  They are able to identify if a participant is able to achieve their goal and identify the future actions that can help achieve their goal.

\paragraph{\textit{Revising plans help with goal achievement.}} 1) Revising in actual stories and 2) revising in counterfactual stories 3) does the state have any affect on revising?




==> sections/unused_results.tex <==

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|l|c|c|c|c|}
 \hline
&& \multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterf.}\\ 
Split&Model&Acc&mF1&Acc&mF1\\
\hline
\multirow{5}{*}{Val} 
& Maj.   &.79&.44&.80&.30 \\ 
& T511b  &.50&.29&.58&.31 \\
& fT5b   &.59&.31&.64&.34 \\
& fT5l   &.26&.24&.61&.33 \\
& fT5xl  &.29&.27&.29&.19 \\
& fT5xxl &.29&.27&.42&.26 \\
& gpt3.5t&.57&.53+&.65&.38+ \\
& gpt4   &.64&.59+&.79&.42+ \\
 \hline
\hline
\multirow{5}{*}{Test} 
& Maj.   &.62&.26&.62&.26 \\ 
& T511b  &.48&.31&.52&.34 \\
& fT5b   &.49&.30&.47&.28 \\
& fT5l   &.45&.31&.43&.28 \\
& fT5xl  &.40&.28&.44&.30 \\
& fT5xxl &.42&.28&.43&.29 \\
& gpt3.5t&.31&.22&.48&.31+ \\
& gpt4   &.44&.30+&.59&.38+ \\
\hline
\end{tabular}
}
 \caption{Identifying whether a revision will help with goal achievement.  }
\label{tab:goals-revision-metrics}
\end{table}

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|l|c|c|c|c|}
 \hline
&& \multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterf.}\\ 
Split&Model&Acc&mF1&Acc&mF1\\
\hline
\multirow{5}{*}{Val} 
& Maj.   &.79&.44&.53&.55 \\ 
& T511b  &.52&.50&.52&.52 \\
& fT5b   &.47&.32&.43&.30 \\
& fT5l   &.67&.40&.59&.59 \\
& fT5xl  &.79&.44&.52&.42 \\
& fT5xxl &.71&.42&.56&.53 \\
& gpt3.5t&.64&.52&.67&.65 \\
& gpt4   &.64&.52&.51&.50 \\
 \hline
\hline
\multirow{5}{*}{Test} 
& Maj.   &.56&.36&.61&.38 \\ 
& T511b  &.53&.53&.54&.54 \\
& fT5b   &.39&.28&.41&.29 \\
& fT5l   &.51&.49&.61&.61 \\
& fT5xl  &.59&.43&.47&.42 \\
& fT5xxl &.60&.50&.53&.51 \\
& gpt3.5t&.53&.49&.58&.57+ \\
& gpt4   &.53&.47&.60&.60+ \\
\hline
\end{tabular}
}
 \caption{Identifying whether achievable goals are revised.}
\label{tab:achievable-goals-revised-metrics}
\end{table}

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|l|c|c|c|c|}
 \hline
&& \multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterf.}\\ 
Split&Model&Acc&mF1&Acc&mF1\\
\hline
\multirow{5}{*}{Val} 
& Maj.   &.79&.44&.80&.45 \\ 
& T511b  &.20&.16&.20&.17 \\
& fT5b   &.79&.44&.59&.42 \\
& fT5l   &.57&.36&.71&.42 \\
& fT5xl  &.79&.44&.80&.45 \\
& fT5xxl &.79&.44&.80&.45 \\
& gpt3.5t&.79&.44&.80&.45 \\
& gpt4   &&&& \\
 \hline
\hline
\multirow{5}{*}{Test} 
& Maj.   &.62&.38&.62&.38 \\ 
& T511b  &.38&.28&.20&.17 \\
& fT5b   &.79&.47&.63&.40 \\
& fT5l   &.56&.67&.60&.50 \\
& fT5xl  &.62&.38&.62&.38 \\
& fT5xxl &.62&.38&.62&.38 \\
& gpt3.5t&.62&.38&.62&.38 \\
& gpt4   &&&& \\
\hline
\end{tabular}
}
 \caption{Identifying Original vs Revised plans by Models }
\label{tab:plan-revision}
\end{table}


\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
 \hline
& \multicolumn{4}{|c|}{Overall Satisfaction} & \multicolumn{4}{|c|}{ Achievement Satisfac.}\\  &\multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterfac.}&\multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterfac.}\\ 
Model&Acc&mF1&Acc&mF1&Acc&F1&Acc&F1\\
\hline
Maj.   &.72&.28&.62&.26&.87&.47&.62&.26\\ 
T511b  &.60&.33&.52&.32&.53&.43&.52&.48  \\
fT5b   &.74&.36&.64&.36   &.89&.67&.73&.54 \\
fT5xxl &.87&.58&.66&.45&.89&.77&.68&.65\\
gpt3.5t&.84&.54&.63&.48&.86&.75&.64&.62 \\
gpt4   &.87&.57&.67&.50&.89&.78&.70&.66 \\
\hline
\end{tabular}
}
\caption{Participant's satisfaction with the state of goal achievement}
\label{tab:goal-satisfaction-metrics}
\end{table}

\begin{table}[t]
\centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|l|c|c|c|c|}
 \hline
&& \multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterf.}\\ 
Split&Model&Acc&mF1&Acc&mF1\\
\hline
\multirow{5}{*}{Val} 
& Maj.   &.89&.47&.78&.44 \\ 
& T511b  &.57&.44&.52&.47 \\
& fT5b   &.88&.59&.73&.45 \\
& fT5l   &.86&.74&.68&.64 \\
& fT5xl  &.88&.68&.81&.75 \\
& fT5xxl &.92&.82&.82&.79 \\
& gpt3.5t&.85&.73&.73&.70 \\
& gpt4   &.88&.72&.82&.78 \\
 \hline
\hline
\multirow{5}{*}{Test} 
& Maj.   &.87&.47&.62&.26 \\ 
& T511b  &.53&.43&.52&.48 \\
& fT5b   &.89&.67&.73&.54 \\
& fT5l   &.81&.70&.59&.57 \\
& fT5xl  &.92&.82&.70&.65 \\
& fT5xxl &.89&.77&.68&.65 \\
& gpt3.5t&.86&.75&.64&.62 \\
& gpt4   &.89&.78&.70&.66 \\
\hline
\end{tabular}
}
\caption{Participant's satisfaction measurement for achievable goals}
\label{tab:goal-satisfaction-with-achievement-metrics}
\end{table}

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|l|c|c|c|c|}
 \hline
&& \multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterf.}\\ 
Split&Model&Acc&mF1&Acc&mF1\\
\hline
\multirow{5}{*}{Val} &
Maj.   &.73&.28&.58&.24 &.62&.38&.48&.22\\ 
 T511b  &.68&.39&.65&.42 &.66&.38&.62&.35\\
 fT5b   &.72&.28&.61&.32 &.59&.42&.54&.32 \\
 fT5xxl &.67&.41&.85&.59 &.75&.47&.80&.55\\
 gpt3.5t&.64&.40&.80&.55 &.67&.42&.74&.54 \\
 gpt4   &.58&.37&.65&.46 &.80&.68&.80&.68\\
 \hline
 T5b-ft &.65&.41&.73&.50 &.72&.42&.70&.49\\
 fT5b-ft&.65&.37&.77&.53 &.74&.44&.72&.50\\
 \hline
 & Maj.    &.73&.28&.58&.24 \\ 
& T511b   &.68&.39&.65&.42 \\
& T5b-ft  &.65&.41&.72&.49 \\
& fT5b    &.72&.28&.61&.32 \\
& fT5b-ft &.65&.37&.77&.53 \\
& fT5l    &.66&.39&.77&.53 \\
& fT5l-ft &.67&.38&.82&.57 \\
& fT5xl   &.64&.39&.82&.57 \\
& fT5xl-ft&.71&.47&.78&.58 \\
& fT5xxl  &.67&.41&.85&.59 \\
& gpt3.5t &.64&.40&.80&.55 \\
& gpt4    &.58&.37&.65&.46 \\
 \hline
\hline
\multirow{5}{*}{Test} 
& Maj.    &.62&.38&.48&.22 \\ 
& T511b   &.66&.38&.62&.35 \\
& T5b-ft  &.72&.42&.72&.49 \\
& fT5b    &.59&.42&.54&.32 \\
& fT5b-ft &.74&.44&.72&.50 \\
& fT5l    &.66&.57&.70&.49 \\
& fT5l-ft &.74&.45&.73&.54 \\
& fT5xl   &.73&.46&.79&.55 \\
& fT5xl-ft&.76&.49&.71&.55 \\
& fT5xxl  &.75&.47&.80&.55 \\
& gpt3.5t &.67&.42&.74&.54 \\
& gpt4    &.80&.68&.80&.68 \\
\hline
\end{tabular}
}
 \caption{Model identification of Goal achievement at the end of a story.  }
\label{tab:all-goals-success-in-story-metrics}
\end{table}
\emph{\textbf{Are larger models better at identifying  participants' satisfaction?}}
A proxy for goal achievement is a participant's satisfaction during and after goal achievement.  We cast identifying satisfaction as an entailment task with the story, goal and next action as premise and ask if the participant is satisfied with their goal achievement with the choices of Yes, No and Unsure.  Since participants may not always be satisfied with achieved goals, or unsatisfied with unachieved goals as mentioned in \cref{sec:prospective-goal-knowledge} we repeat this task with only achieved goals and cast it as a binary inference.  Refer to \cref{tab:task-prompts} for the prompt setup for both variations of the task. The results from this variation are presented in \cref{tab:goal-satisfaction-with-achievement-metrics}.  Performance for both the setups improves with model size. FlanT5's fine-training on a large number of tasks helps on this task as even the base Flan-T5 model performs better than T5-11b. All models perform better for the actual story context than the counterfactual story context.  We attribute this difference to the fact that a goal annotated for an actual story may not perfectly suit the counterfactual story context. 

\begin{table}[t]
 \centering
\resizebox{.68\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|}
 \hline
Model& Goal (F1)& Full Agr. (F1) & Partial A. (F1)\\ 
\hline
Maj.  &.68&.67&.00 \\
%Ref.   &   &.  &.  &.  \\
%T511b   &.47/.36&.47/.26&.52/.38\\
fT5b (0 \& 3-shot)&.51/.60&.55/.62&.48/.59 \\
%ft5l    &.54/.65&.60/.70&.49/.62\\
%ft5xl   &.62/.47&.67/.57&.58/.38\\
fT5xxl (0 \& 3-shot)&.76/.73&.90/.90&.66/.58 \\
gpt3.5t (0-shot)&.63/.56&.78/.76&.53/.39\\
gpt3.5t (3-shot)&.69/.65&.79/.79&.61/.52\\
gpt4  (0-shot)&.76/.72 &.87/.86 &.67/.52 \\
gpt4  (3-shot)&.76/.72&.88/.88&.66/.48\\
\hline
T5b-ft (0-shot)&.58/.69&.63/.72&.54/.66 \\%(epoch 4) 
fT5b-ft (0-shot)&.56/.69&.63/.73&.51/.65 \\%(epoch 1)
fT5b-ft (3-shot)&\textbf{.75/.79}&.85/.87&\textbf{.65/.69}\\%(epoch 1)
\hline
\end{tabular}
}
 \caption{Evaluation of goal transferability comparing performance in full \& partial agreement stories.  %Significantly higher (compared to all other models) are bolded.
 %\todo[inline]{check stat. sign.}
% \todo[inline]{limiting verbosity, state one sentence take-away}
}
\label{tab:counterfactual-applicability-metrics}
\vspace{-5mm}
\end{table}

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
 \hline
 & \multicolumn{5}{|c|}{Actual Story} & \multicolumn{5}{|c|}{Counterfactual Story}\\  Model  & Rou  & ME&P.Type&\multicolumn{2}{|c|}{Human Eval.} & Rou &ME&P.Type&\multicolumn{2}{|c|}{Human Eval.}\\ 
  Type&  L &TR &Acc/F1& Plan &Type&  L &TR&Acc/F1& Plan &Type\\
 \hline
\hline
Ref/Maj    &-&-&.62/.77&4.28&4.28&-&-&.62/.77&4.31&4.29 \\ 
%&&Ref    &&&&&4.25&3.95 &&&&&4.34&4.34\\
fT5b (3-shot)&.19&.24&.47/.37 &\underline{3.5}&\underline{3.21} &.20&.24&.55/.48&\underline{3.09}&\underline{2.85} \\
%&&Ref    &&&&&4.20&4.20 &&&&&4.23&4.23\\
fT5xxl (3-shot)&.22&.24&.52/.44&\underline{3.26}&\underline{2.78}&.20&.23&.52/.38&\underline{3.57}&\underline{2.96}\\
%&&Ref    &&&&4.29&4.29&  &&&&&4.39&4.36\\
gpt3.5t (3-shot)&.19&.25&.75/.83&3.87&\underline{2.35}&.17&.23&.65/.72&3.99&\underline{2.87}\\
%&&Ref    &&&&&4.29&4.23 &&&&&4.37&4.37 \\
gpt4 (3-shot) &.20&.21&.78/.82&4.16&\underline{3.22}&.17&.20&.75/.79&4.07&\underline{2.95}\\
\hline
%%T5b-ft (0-shot) &.16&.11&.70/.78&3.60&\underline{3.16}&.12&.10&.76/.83&4.1&\underline{3.33}\\
fT5b-ft (0-shot)&.16&.10&.72/.79&4.07&\underline{3.15}&.12&.09&.89/.91&3.72&\underline{3.33}\\ 
fT5b-ft (3-shot)&.14&.17&.72/.79&\underline{2.96}&\underline{2.89}&.10&.09&.89/.91&\underline{2.78}&\underline{2.99}\\ 
%fT5l-ft&.16&.12&.75/.82&-&-&.15&.11&.86/.89&-&-\\
\hline
\end{tabular}
}
 \caption{Evaluation of model generated plans and plan types.  Ref/Maj is the majority class accuracy/F1 for the Plan Type and gold label human evaluation scores. Underlined scores are significantly lower than reference. 
%\todo[inline]{work on narrative}
}
\label{tab:future-plan-manual-metrics}
\vspace{-2mm}
\end{table}
\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
 \hline
 & \multicolumn{5}{|c|}{Actual Story} & \multicolumn{5}{|c|}{Counterfactual Story}\\  Model  & Rou  & ME&P.Type&\multicolumn{2}{|c|}{Human Eval.} & Rou &ME&P.Type&\multicolumn{2}{|c|}{Human Eval.}\\ 
  Type&  L &TR &F1& Plan &Type&  L &TR&F1& Plan &Type\\
 \hline
\hline
Ref/Maj    &-&-&.77&4.28&4.28&-&-&.77&4.31&4.29 \\ 
%&&Ref    &&&&&4.25&3.95 &&&&&4.34&4.34\\
fT5b (3-shot)&.19&.24&.37 &\underline{3.5}&\underline{3.21} &.20&.24&.48&\underline{3.09}&\underline{2.85} \\
%&&Ref    &&&&&4.20&4.20 &&&&&4.23&4.23\\
fT5xxl (3-shot)&.22&.24&.44&\underline{3.26}&\underline{2.78}&.20&.23&.38&\underline{3.57}&\underline{2.96}\\
%&&Ref    &&&&4.29&4.29&  &&&&&4.39&4.36\\
gpt3.5t (3-shot)&.19&.25&.83&3.87&\underline{2.35}&.17&.23&.72&3.99&\underline{2.87}\\
%&&Ref    &&&&&4.29&4.23 &&&&&4.37&4.37 \\
gpt4 (3-shot) &.20&.21&.82&4.16&\underline{3.22}&.17&.20&.79&4.07&\underline{2.95}\\
%\hline
%%T5b-ft (0-shot) &.16&.11&.70/.78&3.60&\underline{3.16}&.12&.10&.76/.83&4.1&\underline{3.33}\\
fT5b-ft (0-shot)&.16&.10&.79&4.07&\underline{3.15}&.12&.09&.91&3.72&\underline{3.33}\\ 
%fT5b-ft (3-shot)&.14&.17&.79&\underline{2.96}&\underline{2.89}&.10&.09&.91&\underline{2.78}&\underline{2.99}\\ 
%fT5l-ft&.16&.12&.75/.82&-&-&.15&.11&.86/.89&-&-\\
\hline
\end{tabular}
}
 \caption{Evaluation of model generated plans and plan types.  Ref/Maj is the majority class F1 for Plan Type and gold label human evaluation scores. Underlined scores are significantly lower than reference. Human evaluation examines the correctness of plan and its type.
%\todo[inline]{work on narrative}
}
\label{tab:future-plan-manual-metrics}
\vspace{-2mm}
\end{table}

\begin{table*}[t]
\centering
\resizebox{.98\textwidth}{!}{
 \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c|c|c|}
 \cline{2-14}
  &  & \multicolumn{3}{|c|}{Rouge} & MET- & \multicolumn{2}{|c|}{BLEU} & Bert-&\multicolumn{5}{|c|}{Human Evaluation}\\ 
  & & R1 & R2 & RL & EOR & Corpus & Google & Score&Cohere &Explain & Faith & Truth & Intent\\
 \cline{2-14}
 \cline{2-14}
 &Reference & \multicolumn{7}{|c|}{-} &4.76 & 4.67 & 4.9 & 4.91 & 4.74 \\ 
 \cline{2-14}
\multirow{6}{*}{Val Split} 
& T5-11b  &  &  &  &  &  &  & &&&&& \\
& flanT5b  &  .37  &  .14 & .36 & .34  &  0.9 & .14 &.86& 3.72- & 3.94- &4.15-&3.79- & 3.64-  \\
& flanT5l  & .41  & .22  & .4 & .3  & .16  & .14 & .84 &&&&&\\
& flanT5xl & .42  & .21 & .4 & .33  & .17  & .15 & .85&&&&&\\
& flanT5xxl&  .45 & .25 & .44 & .43  & .2  & .2 & .86 &4.5&4.37&4.86&4.92 &4.38\\
& gpt3.5t  &  .44 & .21 & .42 &  .49 & .11  & .15 & &4.68&\textbf{4.93+}&4.86&4.86&4.42\\
& gpt4     & .5  & .3 & .49 &.51   &.21   & .23 & &4.94&4.9&4.98&4.98&4.86\\
\hline
\multirow{10}{*}{Act.}&\multirow{5}{*}{Val}
 &\multicolumn{3}{|l|}{Ref mean vals (var < \%) }&4.81&4.78 &4.91 &4.97 &4.82 \\ 
&& Ref    &&      &4.73 &4.76 &4.96 &5.00 &4.84 \\
&&fT5b    &.38&.36&\underline{3.61}&\underline{3.85}&\underline{4.20}&\underline{3.69}&\underline{3.52} \\ 
&& Ref    &&      &4.83 &4.79 &4.84 &4.92 &4.75 \\
&& fT5xxl &.44&.44&4.47 &4.43 &4.93 &4.92 &4.37 \\
&& Ref    &&      &4.75 &4.68 &4.87 &5.00 &4.69 \\
&& gpt3.5t&.43&.50&4.67 &\textbf{4.96}&4.84 &4.84 &4.53 \\
&& Ref    &&      &4.92 &4.88 &4.96 &4.96 &4.83 \\
&& gpt4   &.48&.53&4.91 &4.87 &5.00 &5.00 &4.8\\
\cline{2-10}
&\multirow{5}{*}{Test} 
 &\multicolumn{3}{|l|}{Ref mean vals (var < \%) }&4.74&4.69&4.78&4.78&4.49 \\ 
&& Ref    &&      &4.73 &4.67 &4.78 &4.85 &4.43 \\
&& fT5b   &.42&.40&\underline{3.95}&\underline{4.19}&4.50 &\underline{4.35}&\underline{3.72} \\
&& Ref    &&      &4.75 &4.71 &4.77 &4.88 &4.54 \\
&& fT5xxl &.50&.49&4.49 &4.65 &4.83 &4.81 &\underline{4.03} \\
&& Ref    &&      &4.73 &4.65 &4.76 &4.74 &4.49 \\
&& gpt3.5t&.44&.52&4.53 &4.59 &\textbf{4.95}&\underline{3.89}&4.90 \\
&& Ref    &&      &4.75 &4.71 &4.81 &4.81 &4.48 \\
&& gpt4   &.53&.55&\underline{4.46}&4.44 &4.82 &4.82 &\underline{3.92}\\
\hline
\hline
  &Reference & \multicolumn{7}{|c|}{-} &4.74 & 4.73 & 4.79 & 4.83 & 4.57 \\ 
\hline
\multirow{6}{*}{Test Split} 
& T5-11b  &  &  &  &  &  &  & &&&&& \\
& flanT5b & .44 & .21 & .42 & .4 & .11 & .16 & .86 &3.47-&3.78-&4.1-&3.97-&3.32-\\
& flanT5l &.45 & .23 & .45 & .32 & .18 & .15 & .86 &&&&&\\
& flanT5xl  & .47 & .25 & .46 & .36  & .18 & .16 & .86 &&&&&\\
& flanT5xxl  & .50 & .27  & .49 & .46  & .2  & .2 & .86&4.31-&4.47- &4.67&4.71&4.0-\\
& GPT3.5t & .44 & .22 & .42 &  .49&  .1 & .14&&4.47-&4.47-&4.86&4.81&3.9-\\
& GPT4  & .52 & .32 & .51 & .53 & .22 & .24 &  &4.53&4.49&4.81&4.82&4.00-\\
 \hline
 \cline{2-9}
 \end{tabular}
 }
 \caption{Automated and Human Evaluation scores for model generated Goals.\todo[inline]{fix table} }
\label{tab:goal-description-all-metrics}
\end{table*}


\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l||l|l|c|c|c|c|c|}
 \hline
  Story &Split&Model  & Rouge & MET &\multicolumn{3}{|c|}{Human Eval}\\ 
  Type& & & L & EOR & Cohere &Cohesive & Explain \\
 \hline
\hline
\multirow{10}{*}{Act.}&\multirow{5}{*}{Val}
 &Ref & &&4.70&4.64&4.79 \\ 
&&Ref     & &&4.53&4.58&4.5 \\ 
&& fT5b   &.29&.29&\underline{2.06}&\underline{1.64} &\underline{1.17}\\
&&Ref     & &&4.85&4.77&4.92 \\ 
&& fT5xxl &.45&.49&4.77&4.49&\underline{4.24}\\
&&Ref     & &&4.72&4.60&4.88 \\ 
&& gpt3.5t&.40&.46&4.72&4.75&4.88\\
&&Ref     & &&4.68&4.60&4.84 \\ 
&& gpt4   &.45&.48&4.92&\textbf{4.88}&4.96\\
\cline{2-8}
&\multirow{5}{*}{Test} 
 &Ref     &  &&4.68&4.53&4.88 \\ 
&&Ref     & &&4.67&4.58&4.91 \\ 
 && fT5b  &.30&.31 &\underline{2.35}& \underline{2.15} & \underline{1.39}\\
&&Ref     & &&4.58&4.44&4.84 \\ 
&& fT5xxl &.47&.50&4.62&4.54&\underline{3.97}\\
&&Ref     & &&4.77&4.63&4.88 \\ 
&& gpt3.5t&.43&.48&4.85&4.71&4.83\\
&&Ref     & &&4.68&4.49&4.90 \\ 
&& gpt4   &.45&.50&4.87&4.75&4.87\\
\hline
\hline
\multirow{10}{*}{Cou.}&\multirow{5}{*}{Val}
 &Ref     & &&4.55&4.54&4.85 \\ 
&&Ref     & &&4.47&4.59&4.77 \\ 
&& fT5b   &.30&.30&\underline{1.73}&\underline{1.76}&\underline{1.43}\\
&&Ref     & &&4.60&4.40&4.67 \\ 
&& fT5xxl &.45&.49&4.77&4.45&\underline{4.16}\\
&&Ref     & &&4.56&4.52&4.83 \\ 
&& gpt3.5t&.40&.46&\textbf{4.93}&\textbf{4.84}&4.88\\
&&Ref     & &&4.67&4.59&4.83 \\ 
&& gpt4   &.44&.48&4.88&4.88&4.88\\
\cline{2-8}
&\multirow{5}{*}{Test} 
 &Ref     & &&4.71&4.60&4.61 \\ 
&&Ref     & &&4.70&4.55&4.50 \\ 
&& fT5b   &.31&.31&\underline{1.87}&\underline{2.00}&\underline{1.56}\\
&&Ref     & &&4.75&4.55&4.63 \\ 
&& fT5xxl &.47&.49&\underline{3.92}&\underline{3.83}&\underline{3.69}\\
&&Ref     & &&4.79&4.67&4.65 \\ 
&& gpt3.5t&.41&.47&4.79&4.62&4.82\\
&&Ref     & &&4.79&4.63&4.65 \\ 
&& gpt4   &.45&.49&4.63&4.57&\textbf{4.95}\\
\hline
\end{tabular}
}
 \caption{Automated and Human Evaluation scores for model generated Next Actions. \todo[inline]{fix table} }
\label{tab:next-actions-manual-metrics2}
\end{table}

